Enhanced Optical Dichroism of Graphene Nanoribbons

The optical conductivity of graphene nanoribbons is analytical and exactly derived. It is shown that the absence of translation invariance along the transverse direction allows considerable intra-band absorption in a narrow frequency window that varies with the ribbon width, and lies in the THz range domain for ribbons 10-100nm wide. In this spectral region the absorption anisotropy can be as high as two orders of magnitude, which renders the medium strongly dichroic, and allows for a very high degree of polarization (up to ~85) with just a single layer of graphene. The effect is resilient to level broadening of the ribbon spectrum potentially induced by disorder. Using a cavity for impedance enhancement, or a stack of few layer nanoribbons, these values can reach almost 100%. This opens a potential prospect of employing graphene ribbon structures as efficient polarizers in the far IR and THz frequencies.

==> PaxHeader/ribbon_dichroism.tex <==
30 mtime=1346494270.288112218
30 ctime=1346496729.197371622
30 atime=1346494270.335111627
20 SCHILY.dev=64770
22 SCHILY.ino=3539307
18 SCHILY.nlink=1
88 LIBARCHIVE.xattr.security.selinux=dW5jb25maW5lZF91Om9iamVjdF9yOnVzZXJfaG9tZV90OnMwAA

